Multivariate functional group sparse regression: functional predictor selection

In this paper, we propose methods for functional predictor selection and the estimation of smooth functional coefficients simultaneously in a scalar-on-function regression problem under high-dimensional multivariate functional data setting. In particular, we develop two methods for functional group-sparse regression under a generic Hilbert space of infinite dimension. We show the convergence of algorithms and the consistency of the estimation and the selection (oracle property) under infinite-dimensional Hilbert spaces. Simulation studies show the effectiveness of the methods in both the selection and the estimation of functional coefficients. The applications to the functional magnetic resonance imaging (fMRI) reveal the regions of the human brain related to ADHD and IQ.

==> macro_f_cov.tex <==
%------------------------------------%
% Packages
%------------------------------------%
\usepackage{amsmath,amssymb}
\usepackage{graphicx}% Include figure files
\usepackage{caption}
\usepackage{color}% Include colors for document elements
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{float}
%\usepackage{hyperref} % hyperref must be loaded before apacite
\usepackage{natbib}
\usepackage{datetime}

\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{multirow,verbatim}
\usepackage{latexsym, amsbsy, amssymb}
\usepackage{color}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{tikz}
\usepackage{graphicx}
\usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{apacite}

%\bibliographystyle{asa}
%\hypersetup{ colorlinks = true, citecolor = black, urlcolor = blue}
%\usepackage[nolists, nomarkers, figuresfirst]{endfloat}


%--------------------------------%
% Macro
%--------------------------------%

%--------------------------------%
% Title (little customization)
%--------------------------------%
\makeatletter
\def\@maketitle{%
	\newpage
	\null
	\vskip 2em%
	\begin{center}%
		\let \footnote \thanks
		{\LARGE \@title \par}%
		\vskip 1.5em%
		{\large
			\lineskip .5em%
			\begin{tabular}[t]{c}%
				\@author
			\end{tabular}\par}%
		\vskip 1em%
		%{\large \@date}%
	\end{center}%
	\par
	\vskip 1.5em}
\makeatother
%--------------------------------%
% Keywords
\providecommand{\keywords}[1]{\hspace{1cm}\textbf{\textit{Keywords:}} #1}
%--------------------------------%

%--------------------------------%
% MATH- New Commends 
%--------------------------------%
\def\nano{\scriptscriptstyle}
\def\boe{\begin{enumerate}}
	\def\eoe{\end{enumerate}}
\def\dom{\mathrm{dom}}

\newcommand\inner[2]{\langle #1  \rangle \lo {#2}}

\def\ali{&\,}
\newcommand\hii[1]{\hi {(#1)}}
%--------------------------------%
% MATH- Text/Font-Related
%--------------------------------%
\newcommand\ca[1]{{\cal{#1}}}
\newcommand\lo[1]{_{\nano{#1}}}
\newcommand\hi[1]{^{\nano{#1}}}

%\Large
\newfont{\rsfsten}{rsfs10 scaled 1100}
\newfont{\rsfstena}{rsfs10 scaled 800}
%\newfont{\rsfsten}{rsfs10 scaled 1300}
%\newfont{\rsfstena}{rsfs10 scaled 800}
\newfont{\rsfstenb}{rsfs10 scaled 500}
\newcommand{\sten}[1]{\mbox{\rsfsten #1}\,}
\newcommand{\stens}[1]{\mbox{\rsfstena #1}\,}
\newcommand{\stent}[1]{\mbox{\rsfstenb #1}}
\def\tr{\mathrm{tr}}
\def\vec{\mathrm{vec}}
\def\mat{\mathrm{mat}}
\def\sign{\mathrm{sign}}

\def\argmin{\mathrm{argmin}}
\def\argmax{\mathrm{argmax}}
\def\Range{\mathrm{Range}}
\def\Span{\mathrm{Span}}
\def\tr{\mathrm{tr}}
\def\vec{\mathrm{vec}}
\def\mat{\mathrm{mat}}
\def\sign{\mathrm{sign}}
\def\var{\mathrm{var}}
\def\cov{\mathrm{cov}}

\def\ran{\mathrm{ran}}
\def\cran{\overline{\ran}}

\def\spn{{\rm span}}

%--------------------------------%
% Assumption, Lemma, Theorm,  ...
%--------------------------------%
\newtheorem{assumption}{{\bf Assumption}}
\newtheorem{remark}{{\bf Remark}}
\newtheorem{proposition}{{\bf Proposition}}
\newtheorem{lemma}{{\bf Lemma}}
\newtheorem{corollary}{{\bf Corollary}}
\newtheorem{definition}{{\bf Definition}}
\newtheorem{theorem}{{\bf Theorem}}
\newtheorem{conjecture}{{\bf Conjecture}}
\newtheorem{example}{{\bf Example}}
\newtheorem{problem}{{\bf Problem}}
%--------------------------------%
% MATH-Symbols 
%--------------------------------%

\def\Xt{\tilde{X}}
\def\eop{\hfill $\Box$ \\
}
\def\oc{\hi \perp}
\def\imply{\Rightarrow}

\def\tsum{{\textstyle{\sum}}}
\def\tsumijkl{\tsum \lo {i \in \na} \tsum \lo {j \in \na} \tsum \lo {k \in \na} \tsum \lo {\ell \in \na}  }
\def\eqd{\stackrel{\mbox{\tiny $\cal D$}}=}

\def\E{\mathbb{E}}
\def\R{\mathbb R}
\def\S{\mathbb S}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal{H}}}
\def\HT{\H \lo T}
\def\HX{\H \lo X}
\def\HY{\H \lo Y}
%\def\M{{\cal M}}
\def\L{{\cal L}}
\def\M{\mathfrak M}
\def\N{{\mathfrak {N}}}
\def\S{{\mathfrak{S}}}


\def\kappax{\kappa_{\mbox{\tiny $X$}}}
\def\kappat{\kappa_{\mbox{\tiny $T$}}}
\def\kappay{\kappa_{\mbox{\tiny $Y$}}}
\def\Sigmaxx{\Sigma_{\mbox{\tiny $X\!X$}}}
\def\Sigmaxy{\Sigma_{\mbox{\tiny $X\!Y$}}}
\def\Sigmayx{\Sigma_{\mbox{\tiny $Y\!X$}}}
\def\Sigmayh{\Sigma_{\mbox{\tiny $Y\!H$}}}
\def\Sigmahh{\Sigma_{\mbox{\tiny $H\!H$}}}
\def\Sigmahy{\Sigma_{\mbox{\tiny $H\!Y$}}}
\def\Sigmayy{\Sigma_{\mbox{\tiny $Y\!Y$}}}
\def\As{{\mbox{\tiny $A$}}}
\def\Ss{{\mbox{\tiny $S$}}}
\def\Es{{\mbox{\tiny $E$}}}


\def\real{{\mathbb R}}


\def\ka{\kappa}
\def\trans{^{\sf T}}


\def\Sigmaxx{\Sigma_{\mbox{\tiny $X\!X$}}}
\def\Sigmaxy{\Sigma_{\mbox{\tiny $X\!Y$}}}
\def\Sigmayx{\Sigma_{\mbox{\tiny $Y\!X$}}}
\def\Sigmayy{\Sigma_{\mbox{\tiny $Y\!Y$}}}

% power
\def\inv{^{\mbox{\tiny $-1$}}}
\def\mpinv{\hi {\dagger}}
\def\half{^{\mbox{\tiny $\frac{1}{2}$}}}
\def\mhalf{^{\mbox{\tiny $-\frac{1}{2}$}}}

%--------------------------------%
% STAT-Symbols 
%--------------------------------%

\newcommand{\indep}{\;\, \rule[0em]{.03em}{.65em} \hspace{-.45em}
	\rule[-.05em]{.65em}{.03em} \hspace{-.45em}
	\rule[0em]{.03em}{.65em}\;\,}
\def\eqdis{\stackrel{\mbox{\tiny $\sten D$}}{=}}
\def\cip{\stackrel{\mbox{\tiny $P$}}\rightarrow}
\def\cid{\stackrel{\mbox{\tiny $\sten D$}}\longrightarrow}
\def\iid{\stackbin{\mbox{\tiny $i.i.d.$}}\sim}


==> macro_jmlr.tex <==
%------------------------------------%
% Packages
%------------------------------------%
\usepackage{amsmath,amssymb}
\usepackage{graphicx}% Include figure files
\usepackage{caption}
\usepackage{color}% Include colors for document elements
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{float}
%\usepackage{hyperref} % hyperref must be loaded before apacite
\usepackage{natbib}
\usepackage{datetime}

\RequirePackage[OT1]{fontenc}
\RequirePackage{amsthm,amsmath}

%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage{multirow,verbatim}
%\usepackage{latexsym, amsbsy, amssymb}
% \usepackage{color}
% \usepackage[usenames,dvipsnames]{xcolor}
% \usepackage{tikz}
% \usepackage{graphicx}
% \usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{apacite}

%\bibliographystyle{asa}
%\hypersetup{ colorlinks = true, citecolor = black, urlcolor = blue}
%\usepackage[nolists, nomarkers, figuresfirst]{endfloat}


%--------------------------------%
% Macro
%--------------------------------%

%--------------------------------%
% Title (little customization)
%--------------------------------%
% \makeatletter
% \def\@maketitle{%
% 	\newpage
% 	\null
% 	\vskip 2em%
% 	\begin{center}%
% 		\let \footnote \thanks
% 		{\LARGE \@title \par}%
% 		\vskip 1.5em%
% 		{\large
% 			\lineskip .5em%
% 			\begin{tabular}[t]{c}%
% 				\@author
% 			\end{tabular}\par}%
% 		\vskip 1em%
% 		%{\large \@date}%
% 	\end{center}%
% 	\par
% 	\vskip 1.5em}
% \makeatother
%--------------------------------%
% Keywords
\providecommand{\keywords}[1]{\hspace{1cm}\textbf{\textit{Keywords:}} #1}
%--------------------------------%

%--------------------------------%
% MATH- New Commends 
%--------------------------------%
\def\nano{\scriptscriptstyle}
\def\boe{\begin{enumerate}}
	\def\eoe{\end{enumerate}}
\def\dom{\mathrm{dom}}

\newcommand\inner[2]{\langle #1  \rangle \lo {#2}}

\def\ali{&\,}
\newcommand\hii[1]{\hi {(#1)}}
%--------------------------------%
% MATH- Text/Font-Related
%--------------------------------%
\newcommand\ca[1]{{\cal{#1}}}
\newcommand\lo[1]{_{\nano{#1}}}
\newcommand\hi[1]{^{\nano{#1}}}

%\Large
\newfont{\rsfsten}{rsfs10 scaled 1100}
\newfont{\rsfstena}{rsfs10 scaled 800}
%\newfont{\rsfsten}{rsfs10 scaled 1300}
%\newfont{\rsfstena}{rsfs10 scaled 800}
\newfont{\rsfstenb}{rsfs10 scaled 500}
\newcommand{\sten}[1]{\mbox{\rsfsten #1}\,}
\newcommand{\stens}[1]{\mbox{\rsfstena #1}\,}
\newcommand{\stent}[1]{\mbox{\rsfstenb #1}}
\def\tr{\mathrm{tr}}
\def\vec{\mathrm{vec}}
\def\mat{\mathrm{mat}}
\def\sign{\mathrm{sign}}

\def\argmin{\mathrm{argmin}}
\def\argmax{\mathrm{argmax}}
\def\Range{\mathrm{Range}}
\def\Span{\mathrm{Span}}
\def\tr{\mathrm{tr}}
\def\vec{\mathrm{vec}}
\def\mat{\mathrm{mat}}
\def\sign{\mathrm{sign}}
\def\var{\mathrm{var}}
\def\cov{\mathrm{cov}}

\def\ran{\mathrm{ran}}
\def\cran{\overline{\ran}}

\def\spn{{\rm span}}

%--------------------------------%
% Assumption, Lemma, Theorm,  ...
%--------------------------------%
\newtheorem{assumption}{{\bf Assumption}}
\newtheorem{remark}{{\bf Remark}}
\newtheorem{proposition}{{\bf Proposition}}
\newtheorem{lemma}{{\bf Lemma}}
\newtheorem{corollary}{{\bf Corollary}}
\newtheorem{definition}{{\bf Definition}}
\newtheorem{theorem}{{\bf Theorem}}
\newtheorem{conjecture}{{\bf Conjecture}}
\newtheorem{example}{{\bf Example}}
\newtheorem{problem}{{\bf Problem}}
%--------------------------------%
% MATH-Symbols 
%--------------------------------%

\def\Xt{\tilde{X}}
\def\eop{\hfill $\Box$ \\
}
\def\oc{\hi \perp}
\def\imply{\Rightarrow}

\def\tsum{{\textstyle{\sum}}}
\def\tsumijkl{\tsum \lo {i \in \na} \tsum \lo {j \in \na} \tsum \lo {k \in \na} \tsum \lo {\ell \in \na}  }
\def\eqd{\stackrel{\mbox{\tiny $\cal D$}}=}

\def\E{\mathbb{E}}
\def\R{\mathbb R}
\def\S{\mathbb S}
\def\F{{\cal F}}
\def\G{{\cal G}}
\def\H{{\cal{H}}}
\def\HT{\H \lo T}
\def\HX{\H \lo X}
\def\HY{\H \lo Y}
%\def\M{{\cal M}}
\def\L{{\cal L}}
\def\M{\mathfrak M}
\def\N{{\mathfrak {N}}}
\def\S{{\mathfrak{S}}}


\def\kappax{\kappa_{\mbox{\tiny $X$}}}
\def\kappat{\kappa_{\mbox{\tiny $T$}}}
\def\kappay{\kappa_{\mbox{\tiny $Y$}}}
\def\Sigmaxx{\Sigma_{\mbox{\tiny $X\!X$}}}
\def\Sigmaxy{\Sigma_{\mbox{\tiny $X\!Y$}}}
\def\Sigmayx{\Sigma_{\mbox{\tiny $Y\!X$}}}
\def\Sigmayh{\Sigma_{\mbox{\tiny $Y\!H$}}}
\def\Sigmahh{\Sigma_{\mbox{\tiny $H\!H$}}}
\def\Sigmahy{\Sigma_{\mbox{\tiny $H\!Y$}}}
\def\Sigmayy{\Sigma_{\mbox{\tiny $Y\!Y$}}}
\def\As{{\mbox{\tiny $A$}}}
\def\Ss{{\mbox{\tiny $S$}}}
\def\Es{{\mbox{\tiny $E$}}}


\def\real{{\mathbb R}}


\def\ka{\kappa}
\def\trans{^{\sf T}}


\def\Sigmaxx{\Sigma_{\mbox{\tiny $X\!X$}}}
\def\Sigmaxy{\Sigma_{\mbox{\tiny $X\!Y$}}}
\def\Sigmayx{\Sigma_{\mbox{\tiny $Y\!X$}}}
\def\Sigmayy{\Sigma_{\mbox{\tiny $Y\!Y$}}}

% power
\def\inv{^{\mbox{\tiny $-1$}}}
\def\mpinv{\hi {\dagger}}
\def\half{^{\mbox{\tiny $\frac{1}{2}$}}}
\def\mhalf{^{\mbox{\tiny $-\frac{1}{2}$}}}

%--------------------------------%
% STAT-Symbols 
%--------------------------------%

\newcommand{\indep}{\;\, \rule[0em]{.03em}{.65em} \hspace{-.45em}
	\rule[-.05em]{.65em}{.03em} \hspace{-.45em}
	\rule[0em]{.03em}{.65em}\;\,}
\def\eqdis{\stackrel{\mbox{\tiny $\sten D$}}{=}}
\def\cip{\stackrel{\mbox{\tiny $P$}}\rightarrow}
\def\cid{\stackrel{\mbox{\tiny $\sten D$}}\longrightarrow}
\def\iid{\stackbin{\mbox{\tiny $i.i.d.$}}\sim}

